Beyond Worst-case Attacks: Robust RL with Adaptive Defense via Non-dominated Policies

In light of the burgeoning success of reinforcement learning (RL) in diverse real-world applications, considerable focus has been directed towards ensuring RL policies are robust to adversarial attacks during test time. Current approaches largely revolve around solving a minimax problem to prepare for potential worst-case scenarios. While effective against strong attacks, these methods often compromise performance in the absence of attacks or the presence of only weak attacks. To address this, we study policy robustness under the well-accepted state-adversarial attack model, extending our focus beyond only worst-case attacks. We first formalize this task at test time as a regret minimization problem and establish its intrinsic hardness in achieving sublinear regret when the baseline policy is from a general continuous policy class, $\Pi$. This finding prompts us to \textit{refine} the baseline policy class $\Pi$ prior to test time, aiming for efficient adaptation within a finite policy class $\Tilde{\Pi}$, which can resort to an adversarial bandit subroutine. In light of the importance of a small, finite $\Tilde{\Pi}$, we propose a novel training-time algorithm to iteratively discover \textit{non-dominated policies}, forming a near-optimal and minimal $\Tilde{\Pi}$, thereby ensuring both robustness and test-time efficiency. Empirical validation on the Mujoco corroborates the superiority of our approach in terms of natural and robust performance, as well as adaptability to various attack scenarios.

==> fig_all_noswitch_heatmap.tex <==
\begin{figure}[!ht]
    \vspace{-0.3em}
    \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/noswitch/noswitch_none_hm.pdf}
         \caption{Natural}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/noswitch/noswitch_random_hm.pdf}
         \caption{Random}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/noswitch/noswitch_paad_hm.pdf}
         \caption{PA-AD}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \caption{Evolution of bandit weights under no-switch attack.}
\end{figure}

==> fig_all_periodic_heatmap.tex <==
\begin{figure}[!ht]
    \vspace{-0.3em}
    \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_1_hm.pdf}
         \caption{$T=$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_2_hm.pdf}
         \caption{$T=1000$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_4_hm.pdf}
         \caption{$T=500$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_5_hm.pdf}
         \caption{$T=400$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
         \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_8_hm.pdf}
         \caption{$T=250$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_10_hm.pdf}
         \caption{$T=200$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_16_hm.pdf}
         \caption{$T=125$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/periodic/periodic_20_hm.pdf}
         \caption{$T=100$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \caption{Periodic attack.}
\end{figure}

==> fig_all_prob_heatmap.tex <==
\begin{figure}[!ht]
    \vspace{-0.3em}
    \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch/prob_switch_p0.2_hm.pdf}
         \caption{$p=0.2$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch/prob_switch_p0.4_hm.pdf}
         \caption{$p=0.4$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch/prob_switch_p0.5_hm.pdf}
         \caption{$p=0.5$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch/prob_switch_p0.6_hm.pdf}
         \caption{$p=0.6$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
         \centering
     \begin{subfigure}{0.32\textwidth}
     \vspace{-0.2em}
     \centering
        %\subcaption{Period=$$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch/prob_switch_p0.8_hm.pdf}
         \caption{$p=0.8$}
         %\label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \caption{Probabilistic switch attack.}
\end{figure}

==> fig_attacker_training.tex <==
\begin{figure}[!ht]
    \centering
     \begin{subfigure}{0.32\textwidth}
     \centering
        \subcaption{Ant, Natural}
         \includegraphics[width=\linewidth]{./figure/results/ant_none_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \centering
        \subcaption{Ant, Random}
         \includegraphics[width=\linewidth]{./figure/results/ant_random_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}{0.32\textwidth}
     \centering
        \subcaption{Ant, PA-AD}
         \includegraphics[width=\linewidth]{./figure/results/ant_paad_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_attention_ori_paad}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/ant_none_exp3.pdf}
         %\caption{Rewards in Lending}
         \label{fig:bias_infectious_ori_none}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/ant_random_exp3.pdf}
         %\caption{Rewards in Lending}
         \label{fig:bias_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.32\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/ant_paad_exp3.pdf}
         %\caption{Rewards in Lending}
         \label{fig:bias_infectious_ori_paad}
     \end{subfigure}
     \caption{Training attacker}
     
\end{figure}

==> fig_switch_prob.tex <==
\begin{figure}[!ht]
    \centering
     \begin{subfigure}{0.19\textwidth}
     \centering
        \subcaption{$p=0.2$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.2_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
        \subcaption{$p=0.4$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.4_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
        \subcaption{$p=0.5$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.5_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
        \subcaption{$p=0.6$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.6_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
        \subcaption{$p=0.8$}
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.8_hm.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \begin{subfigure}{0.19\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.2_plot.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_attention_ori_natural}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.4_plot.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.5_plot.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.6_plot.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \centering
     \begin{subfigure}[b]{0.19\textwidth}
     \centering
         \includegraphics[width=\linewidth]{./figure/results/prob_switch_p0.8_plot.pdf}
         %\caption{Rewards in Lending}
         \label{fig:rewards_infectious_ori_random}
     \end{subfigure}
     \caption{Evolution of bandit weights and average rewards over rounds under probabilistic switch attack. In the first row of heatmaps, the horizon axis is for time and the vertical axis is for different arms. The cells with lighter color refers to greater weights on this arm. In the second line of plots, the gray zone refers to the rounds where the attacker is active.}
     \label{fig:switch_prob}
\end{figure}

==> table_mujoco_app.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{c|c|p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering}}
\toprule
\textbf{Environment}                  & \textbf{Model}          & \begin{tabular}[c]{@{}c@{}}{\bf Natural}\\{\bf Reward}\end{tabular} & \textbf{Random}      & \textbf{MAD}          & \textbf{RS}          & \textbf{SA-RL}       & \textbf{PA-AD}        \\
 \hline
\multirow{6}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Halfcheetah}}\\state-dim: 17\\$\epsilon$=0.15\end{tabular}}    & PPO (vanilla)    & \textbf{7117 $\pm$ 98}    & 5486 $\pm$ 1378 & 1836 $\pm$ 866  & 489 $\pm$ 758   & -660 $\pm$ 218  & -356 $\pm$ 407     \\  
 & SA-PPO           & 3632 $\pm$ 20      & 3619 $\pm$ 18   & 3624 $\pm$ 23   & 3283 $\pm$ 20   & 3028 $\pm$ 23  & 2512 $\pm$ 16  \\
 & ATLA-PPO            & 6157 $\pm$ 852     & 6164 $\pm$ 603  & 5790 $\pm$ 174  & 4806 $\pm$ 392  & 5058 $\pm$ 418  & 2576 $\pm$ 548  \\
& PA-ATLA-PPO      & 6289 $\pm$ 342     & \textbf{6215 $\pm$ 346}  & \textbf{5961 $\pm$ 253}  & 5226 $\pm$ 114  & 4872 $\pm$ 379  & 3840 $\pm$ 273  \\
& RADIAL-PPO & 4724 $\pm$ 14 & 4731 $\pm$ 42 & 3994 $\pm$ 156 & 3864 $\pm$ 232 & 3253 $\pm$ 131 & 2674 $\pm$ 168\\
& WocaR-PPO & 6032 $\pm$ 68    & 5969 $\pm$ 149  & 5850 $\pm$ 228  & \textbf{5319 $\pm$ 220}  & \textbf{5365 $\pm$ 54}  & 4269 $\pm$ 172  \\
& \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{7095 $\pm$ 88}    & \cellcolor{lightgray}{5667 $\pm$ 1265}  & \cellcolor{lightgray}{4732 $\pm$ 144}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{5089 $\pm$ 86}  & \cellcolor{lightgray}{\textbf{4428 $\pm$ 471}}  \\
\midrule
\multirow{6}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Hopper} }\\state-dim: 11\\$\epsilon$=0.075\end{tabular}}    & PPO (vanilla)    & 3167 $\pm$ 542      & 2101 $\pm$ 793  & 1410 $\pm$ 655  & 794 $\pm$ 238   & 636 $\pm$ 9  & 160 $\pm$ 136     \\
 & SA-PPO           & 3705 $\pm$ 2     & 2710 $\pm$ 801  & 2652 $\pm$ 835  & 1130 $\pm$ 42     & 1076 $\pm$ 791    & 856 $\pm$ 21  \\
 & ATLA-PPO            & 3291 $\pm$ 600    & 3165 $\pm$ 576  & 2814 $\pm$ 725  & 2244 $\pm$ 618  & 1772 $\pm$ 802 & 1232 $\pm$ 350  \\
& PA-ATLA-PPO      & 3449 $\pm$ 237      & 3325 $\pm$ 239  & 3145 $\pm$ 546  & 3002 $\pm$ 329  & 1529 $\pm$ 284   & 2521 $\pm$ 325  \\
& RADIAL-PPO & \textbf{3740 $\pm$ 44} & \textbf{3729 $\pm$ 100} & 3214 $\pm$ 142 & 2141 $\pm$ 232 & 1722 $\pm$ 186 & 1439  $\pm$ 204\\
 & WocaR-PPO & 3616 $\pm$ 99     & 3633 $\pm$ 30   & \textbf{3541 $\pm$ 207}  & \textbf{3277 $\pm$ 159}  & 2390 $\pm$ 145   & 2579 $\pm$ 229  \\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{3652 $\pm$ 108} & \cellcolor{lightgray}{3585 $\pm$ 179}   & \cellcolor{lightgray}{2825 $\pm$ 819}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{2526 $\pm$ 682}}   & \cellcolor{lightgray}{\textbf{2906 $\pm$ 1059}}  \\
 \midrule
\multirow{6}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Walker2d}}\\state-dim: 17\\$\epsilon$=0.05\end{tabular}}    & PPO (vanilla)    & 4472 $\pm$ 635     & 3007 $\pm$ 1200 & 2869 $\pm$ 1271 & 1336 $\pm$ 654  & 1086 $\pm$ 516    & 804 $\pm$ 130     \\
 & SA-PPO           & 4487 $\pm$ 61      & 4465 $\pm$ 39  & 3668 $\pm$ 689  & 3808 $\pm$ 138  & 2908 $\pm$ 336  & 1042 $\pm$ 353  \\
 & ATLA-PPO            & 3842 $\pm$ 475     & 3927 $\pm$ 368  & 3836 $\pm$ 492  & 3239 $\pm$ 294  & 3663 $\pm$ 707  & 1224 $\pm$ 770  \\
& PA-ATLA-PPO      & 4178 $\pm$ 529     & 4129 $\pm$ 78   & 4024 $\pm$ 272  & 3966 $\pm$ 307  & 3450 $\pm$ 178  & 2248 $\pm$ 131  \\
& RADIAL-PPO & 5251 $\pm$ 12 & 5184 $\pm$ 42 &  4494 $\pm$ 150  & 3572  $\pm$ 239 & 3320 $\pm$ 245 & 1395  $\pm$ 194\\
 & WocaR-PPO & 4156 $\pm$ 495     & 4244 $\pm$ 157  & 4177 $\pm$ 176  & 4093 $\pm$ 138  & 3770 $\pm$ 196  & \textbf{2722 $\pm$ 173}  \\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{6319 $\pm$ 31}} & \cellcolor{lightgray}{\textbf{6309 $\pm$ 36}}  & \cellcolor{lightgray}{\textbf{6292 $\pm$ 57}}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{6085 $\pm$ 620}}  & \cellcolor{lightgray}{\textbf{5930 $\pm$ 1031}}  \\
 \midrule
 \multirow{6}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Ant}}\\state-dim: 111\\$\epsilon$=0.15\end{tabular}}    & PPO (vanilla)    & \textbf{5687 $\pm$ 758}     & 5261 $\pm$ 1005 & 1759 $\pm$ 828 & 268 $\pm$ 227  & -872 $\pm$ 436   & -2580 $\pm$ 872     \\
 & SA-PPO           & 4292 $\pm$ 384     & 4986 $\pm$ 452  & 4662 $\pm$ 522  & 3412 $\pm$ 1755 & 2511 $\pm$ 1117 & -1296 $\pm$ 923  \\
 & ATLA-PPO            & 5359 $\pm$ 153     & 5366 $\pm$ 104  & 5240 $\pm$ 170  & 4136 $\pm$ 149  & 3765 $\pm$ 101  & 220 $\pm$ 338  \\
& PA-ATLA-PPO      & 5469 $\pm$ 106     & 5496 $\pm$ 158  & \textbf{5328 $\pm$ 196}  & 4124 $\pm$ 291  & 3694 $\pm$ 188  & 2986 $\pm$ 364  \\
& RADIAL-PPO & 5076 $\pm$ 254 & 5031 $\pm$ 142 & 4777 $\pm$ 156 & 3731 $\pm$ 177 & 3188 $\pm$ 115 & 1544 $\pm$ 194\\
 & WocaR-PPO & 5596 $\pm$ 225  & \textbf{5558 $\pm$ 241}  & 5284 $\pm$ 182  & \textbf{4339 $\pm$ 160}  & \textbf{3822 $\pm$ 185}  & \textbf{3164 $\pm$ 163}  \\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{5769 $\pm$ 290}} & \cellcolor{lightgray}{5537 $\pm$ 769}  & \cellcolor{lightgray}{4679 $\pm$ 110}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{4524 $\pm$ 79}}  & \cellcolor{lightgray}{\textbf{4338 $\pm$ 161}}  \\
\bottomrule
\end{tabular}}
% \vspace{-1em}
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes on five baselines and on Hopper, Walker2d, Halfcheetah, and Ant. Natural reward and rewards under five types of attacks are reported. Under each column corresponding to an evaluation metric, we bold the best results. And the row for the most robust agent is highlighted as \colorbox{lightgray}{gray}. Note that \textit{ATLA-PPO, PA-ATLA-PPO and RADIAL-PPO are trained with more than $2\times$ steps than}, as reported in.}
\label{tab:mujoco_app}
\vspace{-0.5em}
\end{table*}


==> table_mujoco_app_new.tex <==
\begin{table*}[!t]
\vspace{-0.5em}
\centering
\renewcommand{\arraystretch}{1.2}
\resizebox{\textwidth}{!}{%
\setlength{\tabcolsep}{4pt}
% \setlength{\arrayrulewidth}{1pt}
\begin{tabular}{c|c|p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering} p{2cm}<{\centering}}
\toprule
\textbf{Environment}                  & \textbf{Model}          & \begin{tabular}[c]{@{}c@{}}{\bf Natural}\\{\bf Reward}\end{tabular} & \textbf{Random}      & \textbf{MAD}          & \textbf{RS}          & \textbf{SA-RL}       & \textbf{PA-AD}        \\
 \hline
\multirow{3}{5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Halfcheetah}}\\state-dim: 17\\$\epsilon$=0.15\end{tabular}}
& PA-ATLA-PPO & 6275 $\pm$ 141 & 6137 $\pm$ 117 & 5757 $\pm$ 196 & $\pm$
& $\pm$ & 5187 $\pm$ 486  \\
& WocaR-PPO & 6262 $\pm$ 188 & \textbf{6245 $\pm$ 188} & \textbf{5828 $\pm$ 161} & $\pm$ & $\pm$ & 4406 $\pm$ 1636\\
& \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{7095 $\pm$ 88}}    & \cellcolor{lightgray}{5667 $\pm$ 1265}  & \cellcolor{lightgray}{4732 $\pm$ 144}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{ $\pm$ }}  & \cellcolor{lightgray}{\textbf{ $\pm$ }}  \\
\midrule
\multirow{3}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Hopper} }\\state-dim: 11\\$\epsilon$=0.075\end{tabular}}
& PA-ATLA-PPO & 3594 $\pm$ 31 & 3527 $\pm$ 341 & 2866 $\pm$ 847 & $\pm$ & $\pm$ & 1810 $\pm$ 700 \\
& WocaR-PPO & 3624 $\pm$ 98 & 3568 $\pm$ 207 & \textbf{3056 $\pm$ 764} & $\pm$ & $\pm$ & 2518 $\pm$ 912\\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{3652 $\pm$ 108}} & \cellcolor{lightgray}{\textbf{3585 $\pm$ 179}}   & \cellcolor{lightgray}{2825 $\pm$ 819}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{$\pm$}}   & \cellcolor{lightgray}{\textbf{2906 $\pm$ 1059}}  \\
 \midrule
\multirow{3}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Walker2d}}\\state-dim: 17\\$\epsilon$=0.05\end{tabular}}
& PA-ATLA-PPO & 2430 $\pm$ 1642 & 2088 $\pm$ 1452 & 2414 $\pm$ 1497 & $\pm$ & $\pm$ & $\pm$ \\
& WocaR-PPO & 4132 $\pm$ 957 & 4441 $\pm$ 779 & 4246 $\pm$ 905 & $\pm$ & $\pm$ & 2613 $\pm$ 944\\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{6319 $\pm$ 31}} & \cellcolor{lightgray}{\textbf{6309 $\pm$ 36}}  & \cellcolor{lightgray}{\textbf{6292 $\pm$ 57}}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{5930 $\pm$ 1031}}  \\
 \midrule
 \multirow{3}{5.5em}{\begin{tabular}[c]{@{}c@{}}{\textbf{Ant}}\\state-dim: 111\\$\epsilon$=0.15\end{tabular}}
& PA-ATLA-PPO & 5121 $\pm$ 480 & 4821 $\pm$ 1018 & 4768 $\pm$ 586 & $\pm$ & $\pm$ & 2864 $\pm$ 1592  \\
& WocaR-PPO & 4132 $\pm$ 192 & \textbf{5439 $\pm$ 312} & \textbf{5342 $\pm$ 266} & $\pm$ & $\pm$ & 2903 $\pm$ 112\\
 & \cellcolor{lightgray}{\textbf{Ours}} & \cellcolor{lightgray}{\textbf{5769 $\pm$ 290}} & \cellcolor{lightgray}{5368 $\pm$ 1009}  & \cellcolor{lightgray}{4679 $\pm$ 110}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{$\pm$}}  & \cellcolor{lightgray}{\textbf{4338 $\pm$ 161}}  \\
 
\bottomrule
\end{tabular}}
% \vspace{-1em}
\caption{Average episode rewards $\pm$ standard deviation over 50 episodes on five baselines and ours on Hopper, Walker2d, Halfcheetah, and Ant. Natural reward and rewards under five types of attacks are reported. Under each column corresponding to an evaluation metric, we bold the best results. And the row for the most robust agent is highlighted as \colorbox{lightgray}{gray}. Note that \textit{ATLA-PPO, PA-ATLA-PPO and RADIAL-PPO are trained with more than $2\times$ steps than ours}, as reported in Table.}
\label{tab:mujoco_app}
\vspace{-0.5em}
\end{table*}

